Scalar conservation laws with stochastic discontinuous flux function

A variety of real-world applications are modeled via hyperbolic conservation laws. To account for uncertainties or insufficient measurements, random coefficients may be incorporated. These random fields may depend discontinuously on the state space, e.g., to represent permeability in a heterogeneous or fractured medium. We introduce a suitable admissibility criterion for the resulting stochastic discontinuous-flux conservation law and prove its well-posedness. Therefore, we ensure the pathwise existence and uniqueness of the corresponding deterministic setting and present a novel proof for the measurability of the solution, since classical approaches fail in the discontinuous-flux case. As an example of the developed theory, we present a specific advection coefficient, which is modeled as a sum of a continuous random field and a pure jump field. This random field is employed in the stochastic conservation law, in particular a stochastic Burgers' equation, for numerical experiments. We approximate the solution to this problem via the Finite Volume method and introduce a new meshing strategy that accounts for the resulting standing wave profiles caused by the flux-discontinuities. The ability of this new meshing method to reduce the sample-wise variance is demonstrated in numerous numerical investigations.

==> latex/commands.tex <==
\newcommand{\cred}{\color{red}}
\newcommand{\cblue}{\color{blue}}
\newcommand{\cblack}{\color{black}}
\newcommand{\cgreen}{\color{green}}
\definecolor{bluefromheader}{cmyk}{.83,.44,0,.33} 
\newcommand{\dc}{\color{bluefromheader}}

\makeatletter
\newcommand{\mylabel}[2]{#2\def\@currentlabel{#2}\label{#1}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorem-like environment shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% User shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\LB}[1]{\textcolor{blue}{LB: #1}}
\newcommand{\TODO}[1]{\textbf{\textcolor{red}{ TODO: #1}}}
\newcommand{\highlight}[1]{\textbf{\textcolor{CD03}{#1}}}
\newcommand{\changed}[2]{\textcolor{Plum}{\sout{#1}{#2}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% shortcuts for variables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ball}{\cB}
\newcommand{\charFunc}{\mathds{1}}

\newcommand{\stochDomain}{\Omega}
\newcommand{\sigmaAlgebra}{\cA}
\newcommand{\probSpace}{(\stochDomain, \sigmaAlgebra, \bbP)}
\newcommand{\timeInterval}{\bbT}
\newcommand{\spaceDomain}{\bbX}
\newcommand{\stopTime}{T}
\newcommand{\solFlux}{f}
\newcommand{\fluxFunction}{\mathfrak{\solFlux}}
\newcommand{\invFlux}{\fluxFunction^{-1}_{\pm}}
\newcommand{\spaceVar}{x}
\newcommand{\timeVar}{t}
\newcommand{\stochVar}{\omega}
\newcommand{\solution}{u}
\newcommand{\initialCond}{\solution_{0}}
\newcommand{\steadyStatePar}{\alpha}
\newcommand{\entropyConstant}{m}
\newcommand{\steadyStateSolution}[1]{\entropyConstant^{#1}_{\steadyStatePar}(\spaceVar)}
\newcommand{\steadyStateSolutions}{\entropyConstant^{\pm}_{\steadyStatePar}(\spaceVar)}
\newcommand{\stochSteadyStateSolutions}{\entropyConstant^{\pm}_{\steadyStatePar}(\stochVar, \spaceVar)}
\newcommand{\stochSteadyStateSolution}[1]{\entropyConstant^{#1}_{\steadyStatePar}}
\newcommand{\stochSteadyStateSolutionArg}[1]{\entropyConstant^{#1}_{\steadyStatePar}(\stochVar, \spaceVar)}
\newcommand{\partAdaptedEntropies}[1]{E_{#1}}
\newcommand{\nullSet}{\cN}
\newcommand{\subsolution}{g_{-}}
\newcommand{\supersolution}{g_{+}}
\newcommand{\modalityPointFct}{\solution_M}
\newcommand{\imageBound}{M_0}
\newcommand{\alternativeSolution}{\bar{u}}
\newcommand{\alternativeInitialCond}{\alternativeSolution_{0}}
\newcommand{\lipschitzInterval}{I}
\newcommand{\fluxLipschitzConstant}{L_{\lipschitzInterval}}

\newcommand{\solutionSpace}{L^{\infty}(\bbR \times \timeInterval) \cap C^{0}(\timeInterval; L^{1}_{\text{loc}}(\bbR))}

\newcommand{\altSolution}{v}
\newcommand{\altFluxFunction}{\mathfrak{g}}
\newcommand{\altInitialCond}{\altSolution_{0}}
\newcommand{\solutionInterval}{I}
\newcommand{\doubleAltSol}{\tilde{\altSolution}}
\newcommand{\doubleSol}{\tilde{\solution}}
\newcommand{\globalDomain}{\cD_{\timeInterval}}

\newcommand{\jumpCoeff}{a}
\newcommand{\meanField}{\bar{\jumpCoeff}}
\newcommand{\gaussFunctional}{\phi}
\newcommand{\gaussField}{W}
\newcommand{\jumpField}{P}
\newcommand{\covarianceOperator}{Q}
\newcommand{\borelSigmaAlgebra}{\cB}
\newcommand{\partition}{\cT}
\newcommand{\jumpMeasure}{\lambda}
\newcommand{\domainOfInterest}{\spaceDomain}
\newcommand{\leftDomainBound}{\domainOfInterest_{l}}
\newcommand{\rightDomainBound}{\domainOfInterest_{r}}
\newcommand{\numberOfJumps}{\tau}
\newcommand{\jumpHeights}[1]{\jumpField_{#1}}
\newcommand{\coeffLowerBound}{\jumpCoeff_{-}}
\newcommand{\coeffUpperBound}{\jumpCoeff_{+}}
\newcommand{\discontinuitySet}{\mathfrak{D}}
\newcommand{\jumpPosition}[1]{\chi_{#1}}

\newcommand{\af}{\jumpCoeff_{\fluxFunction}}
\newcommand{\ag}{\jumpCoeff_{\altFluxFunction}}
\newcommand{\f}{f}
\newcommand{\g}{g}

\newcommand{\eigenValue}{\eta}
\newcommand{\eigenFunction}{e}
\newcommand{\KLRV}{Z}
\newcommand{\KLindex}{N}
\newcommand{\approxGaussField}{\gaussField^{\KLindex}_{\bbR}}
\newcommand{\maternAbbrev}{M}

\newcommand{\testFunction}{\varphi}
\newcommand{\variance}{\sigma^2}
\newcommand{\smoothness}{\nu}
\newcommand{\correlationLength}{\rho}
\newcommand{\besselFunction}{K_{\smoothness}}
\newcommand{\hilbertSpace}{H}

\newcommand{\discretization}{\Delta}
\newcommand{\spaceGrid}{\spaceDomain_{\discretization}}
\newcommand{\gridPoint}[1]{\spaceVar_{#1}}
\newcommand{\numGridPoints}{N_{\spaceVar}}
\newcommand{\gridCell}[1]{\cX_{#1}}
\newcommand{\spaceIdx}{i}
\newcommand{\spaceStepSize}[1]{\discretization_{\spaceVar}^{#1}}
\newcommand{\timeGrid}{\timeInterval_{\discretization}}
\newcommand{\timePoint}[1]{\timeVar^{#1}}
\newcommand{\numTimePoints}{N_{\timeVar}}
\newcommand{\timeStepSize}[1]{\discretization_{\timeVar}^{#1}}
\newcommand{\timeCell}[1]{\cT^{#1}}
\newcommand{\timeIdx}{n}
\newcommand{\discontinuityInterface}[1]{d_{#1}}
\newcommand{\waveCell}[1]{\mathfrak{w}_{#1}}

\newcommand{\CFLconst}{L_u^n}

\newcommand{\approxSolution}[2]{\tilde{\solution}^{#1}_{#2}}
\newcommand{\approxFlux}{F}
\newcommand{\inFlux}[2]{\approxFlux^{#1}_{#2-\frac{1}{2}}}
\newcommand{\outFlux}[2]{\approxFlux^{#1}_{#2+\frac{1}{2}}}
\newcommand{\optVar}{\theta}

\newcommand{\smoothingVar}{\varepsilon}
\newcommand{\smoothSolution}{\solution^{\smoothingVar}}
\newcommand{\smoothFluxFunction}{\fluxFunction^{\smoothingVar}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Math operator shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\DeclareAutoPairedDelimiter}[3]{%
  \expandafter\DeclarePairedDelimiter\csname Auto\string#1\endcsname{#2}{#3}%
  \begingroup\edef\x{\endgroup
    \noexpand\DeclareRobustCommand{\noexpand#1}{%
      \expandafter\noexpand\csname Auto\string#1\endcsname*}}%
  \x}

\DeclareAutoPairedDelimiter{\abs}{\lvert}{\rvert}
\DeclareAutoPairedDelimiter{\norm}{\lVert}{\rVert}
\DeclareAutoPairedDelimiter{\set}{\{}{\}}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\expectationOperator}{\bbE}
\newcommand{\expectation}[1]{\expectationOperator \left( #1 \right)}
\newcommand{\timeDeriv}{\frac{\partial}{\partial \timeVar}}
\newcommand{\spaceDeriv}{\frac{\partial}{\partial \spaceVar}}

\renewcommand{\d}[1]{\ensuremath{\operatorname{d}\!{#1}}}
\renewcommand{\div}{\ensuremath{\operatorname{div}}}

\newcommand{\converges}[1]{\ensuremath{\xrightarrow{#1}}}

\DeclareMathOperator*{\esssup}{ess\,sup}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Calligraphic shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Blackboard bold shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

==> latex/packages.tex <==
\usepackage{enumerate}
\usepackage[shortlabels]{enumitem}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{multirow}
\usepackage[firstinits=true]{biblatex}

\usepackage{hyperref}

\usepackage{algorithm,algorithmic}
\newcommand\mycite[1]{{\scriptsize\cite{#1}}}

\usepackage{psfrag}
\usepackage{fullpage}
\usepackage[dvipsnames]{xcolor}
\usepackage{float}

% stroked text
\usepackage[normalem]{ulem}

\usepackage{multicol}
\usepackage{epstopdf}
\usepackage{mathtools}

\usepackage{dsfont}

%\usepackage{caption}
\usepackage{subcaption}

% nice eps figures
\usepackage[process=auto, crop=pdfcrop]{pstool}

% -------- Matlab2Tikz packages -----------------------
\usepackage{pgfplots}
  \pgfplotsset{compat=newest}
  %% the following commands are needed for some matlab2tikz features
  \usetikzlibrary{plotmarks}
  \usetikzlibrary{arrows.meta}
  \usepgfplotslibrary{patchplots}
  \usepackage{grffile}
  \usepackage{amsmath}


==> pictures/GaussianInfluence/correlationLength_L1.tex <==
\begin{figure}[h!tbp]
	\centering
	\begin{subfigure}[b]{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/GaussianInfluence/correlationLength_L1/correlationLength-0-01_L1}{
		\psfrag{95confidenceInterval}{\tiny $95\%$ conf. interval}
		\psfrag{supportLine0.71}{\tiny supp. line with slope $0.71$}
		\psfrag{linearFit0.6}{\tiny lin. fit with slope $0.6$}
		\psfrag{jump-adaptedL1Error}{\tiny avg. strong $L^{1}$ error}
		}
		\caption{Correlation length $\correlationLength = 0.01$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/GaussianInfluence/correlationLength_L1/correlationLength-0-05_L1}{
		\psfrag{95confidenceInterval}{\tiny $95\%$ conf. interval}
		\psfrag{supportLine0.87}{\tiny supp. line with slope $0.87$}
		\psfrag{linearFit0.72}{\tiny lin. fit with slope $0.72$}
		\psfrag{jump-adaptedL1Error}{\tiny avg. strong $L^{1}$ error}
		}
		\caption{Correlation length $\correlationLength = 0.05$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/GaussianInfluence/correlationLength_L1/correlationLength-0-1_L1}{
		\psfrag{95confidenceInterval}{\tiny $95\%$ conf. interval}
		\psfrag{supportLine1}{\tiny supp. line with slope $1.0$}
		\psfrag{linearFit0.84}{\tiny lin. fit with slope $0.84$}
		\psfrag{jump-adaptedL1Error}{\tiny avg. strong $L^{1}$ error}
		}
		\caption{Correlation length $\correlationLength = 0.1$.}
	\end{subfigure}
	\caption{Convergence of the finite volume approximation for different correlation length $\correlationLength$ of the Mat{\'e}rn covariance kernel. The error estimation is based on $20$ samples.}
	\label{fig:Gaussian_correlationLength}
\end{figure}

==> pictures/GaussianInfluence/correlationLength_L1L2.tex <==
\begin{figure}[h!tbp]
	\centering
	\begin{subfigure}[b]{.32\textwidth}
		\psfragfig[width=.38\textwidth]{./pictures/GaussianInfluence/correlationLength_L1L2/correlationLength-0-01_L1L2}{
		\psfrag{95confidenceInterval}{\tiny $95\%$ conf. interval}
		\psfrag{supportLine0.71}{\tiny supp. line with slope $0.71$}
		\psfrag{supportLine0.59}{\tiny supp. line with slope $0.59$}
		\psfrag{linearFit0.48}{\tiny lin. fit with slope $0.48$}
		\psfrag{linearFit0.6}{\tiny lin. fit with slope $0.6$}
		\psfrag{jump-adaptedL1Error}{\tiny avg. strong $L^{1}$ error}
		\psfrag{nonAdaptedL2Error}{\tiny avg. strong $L^{2}$ error}
		}
		\caption{Correlation length $\correlationLength = 0.01$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{.32\textwidth}
		\psfragfig[width=.38\textwidth]{./pictures/GaussianInfluence/correlationLength_L1L2/correlationLength-0-05_L1L2}{
		\psfrag{95confidenceInterval}{\tiny $95\%$ conf. interval}
		\psfrag{supportLine0.87}{\tiny supp. line with slope $0.87$}
		\psfrag{supportLine0.62}{\tiny supp. line with slope $0.62$}
		\psfrag{linearFit0.72}{\tiny lin. fit with slope $0.72$}
		\psfrag{linearFit0.51}{\tiny lin. fit with slope $0.51$}
		\psfrag{jump-adaptedL1Error}{\tiny avg. strong $L^{1}$ error}
		\psfrag{nonAdaptedL2Error}{\tiny avg. strong $L^{2}$ error}
		}
		\caption{Correlation length $\correlationLength = 0.05$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{.32\textwidth}
		\psfragfig[width=.38\textwidth]{./pictures/GaussianInfluence/correlationLength_L1L2/correlationLength-0-1_L1L2}{
		\psfrag{95confidenceInterval}{\tiny $95\%$ conf. interval}
		\psfrag{supportLine1}{\tiny supp. line with slope $1.0$}
		\psfrag{supportLine0.67}{\tiny supp. line with slope $0.67$}
		\psfrag{linearFit0.84}{\tiny lin. fit with slope $0.84$}
		\psfrag{linearFit0.56}{\tiny lin. fit with slope $0.56$}
		\psfrag{jump-adaptedL1Error}{\tiny avg. strong $L^{1}$ error}
		\psfrag{nonAdaptedL2Error}{\tiny avg. strong $L^{2}$ error}
		}
		\caption{Correlation length $\correlationLength = 0.1$.}
	\end{subfigure}
	\caption{Convergence of the finite volume approximation for different correlation length $\correlationLength$ of the Mat{\'e}rn covariance kernel. The error estimation is based on $20$ samples.}
	\label{fig:Gaussian_correlationLength}
\end{figure}

==> pictures/GaussianInfluence/smoothness_L1.tex <==
\begin{figure}[h!tbp]
	\centering
	\begin{subfigure}[b]{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/GaussianInfluence/smoothness_L1/smoothness-0-5}{
		\psfrag{95confidenceInterval}{\tiny $95\%$ conf. interval}
		\psfrag{supportLine0.68}{\tiny supp. line with slope $0.68$}
		\psfrag{linearFit0.62}{\tiny lin. fit with slope $0.62$}
		\psfrag{jump-adaptedL1Error}{\tiny avg. strong $L^{1}$ error}
		}
		\caption{Mat{\'e}rn smoothness $\smoothness = 0.5$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/GaussianInfluence/smoothness_L1/smoothness-1}{
		\psfrag{95confidenceInterval}{\tiny $95\%$ conf. interval}
		\psfrag{supportLine0.78}{\tiny supp. line with slope $0.78$}
		\psfrag{linearFit0.7}{\tiny lin. fit with slope $0.7$}
		\psfrag{jump-adaptedL1Error}{\tiny avg. strong $L^{1}$ error}
		}
		\caption{Mat{\'e}rn smoothness $\smoothness = 1$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/GaussianInfluence/smoothness_L1/smoothness-infty}{
		\psfrag{95confidenceInterval}{\tiny $95\%$ conf. interval}
		\psfrag{supportLine1}{\tiny supp. line with slope $1.0$}
		\psfrag{linearFit0.84}{\tiny lin. fit with slope $0.84$}
		\psfrag{jump-adaptedL1Error}{\tiny avg. strong $L^{1}$ error}
		}
		\caption{Mat{\'e}rn smoothness $\smoothness = \infty$.}
	\end{subfigure}
	\caption{Convergence of the finite volume approximation for different smoothness parameters $\smoothness$ of the Mat{\'e}rn covariance kernel. The error estimation is based on $20$ samples.}
	\label{fig:Gaussian_smoothness}
\end{figure}

==> pictures/coefficientSamples/PoissonSquaredExponential.tex <==
\begin{figure}[h!tbp]
	\centering
	\begin{subfigure}[b]{0.495\textwidth}
		\centering
		\psfragfig[width=0.47\textwidth]{./pictures/coefficientSamples/PoissonSquaredExponential/PoissonSquaredExponential-Sample-1}{
		\psfrag{0}[Bc][Bc]{\hspace*{-10pt}\raisebox{-3pt}{\footnotesize $0$}}
		\psfrag{0.1}{}
		\psfrag{0.2}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.2$}}
		\psfrag{0.3}{}
		\psfrag{0.4}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.4$}}
		\psfrag{0.5}{}
		\psfrag{0.6}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.6$}}
		\psfrag{0.7}{}
		\psfrag{0.8}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.8$}}
		\psfrag{0.9}{}
		\psfrag{1}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $1$}}
		\psfrag{10}[cr][cr]{\raisebox{-3pt}{\footnotesize $10$}}
		\psfrag{20}[cr][cr]{\raisebox{-3pt}{\footnotesize $20$}}
		\psfrag{domain}[Bc][Bc]{\raisebox{-7pt}{spatial domain $\bbX$}}
		\psfrag{coefficient}[bc][tc]{\raisebox{-24pt}{$\jumpCoeff (\stochVar, \spaceVar)$}}
		}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.495\textwidth}
		\centering
		\psfragfig[width=0.47\textwidth]{./pictures/coefficientSamples/PoissonSquaredExponential/PoissonSquaredExponential-Sample-2}{
		\psfrag{x0.0}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0$}}
		\psfrag{x0.2}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.2$}}
		\psfrag{x0.4}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.4$}}
		\psfrag{x0.6}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.6$}}
		\psfrag{x0.8}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.8$}}
		\psfrag{x1.0}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $1$}}
		\psfrag{y0.0}[cr][cr]{\raisebox{-3pt}{\footnotesize $0$}}
		\psfrag{y5.0}[cr][cr]{\raisebox{-3pt}{\footnotesize $5$}}
		\psfrag{y10.0}[cr][cr]{\raisebox{-3pt}{\footnotesize $10$}}
		\psfrag{y15.0}[cr][cr]{\raisebox{-3pt}{\footnotesize $15$}}
		\psfrag{domain}[Bc][Bc]{\raisebox{-7pt}{spatial domain $\bbX$}}
		\psfrag{coefficient}[Bc][Bc]{\raisebox{-0pt}{$\jumpCoeff (\stochVar, \spaceVar)$}}
		}
	\end{subfigure}
	\caption{Two realizations of the Poisson jump field with squared-exponential Gaussian random field.}
	\label{fig:PoissonSquaredExponential_samples}
\end{figure}

==> pictures/coefficientSamples/alternatingExponential.tex <==
\begin{figure}[h!tbp]
	\centering
	\begin{subfigure}[b]{0.495\textwidth}
		\centering
		\psfragfig[width=0.47\textwidth]{./pictures/coefficientSamples/alternatingExponential/alternatingExponential-Sample-1}{
		\psfrag{0}[Bc][Bc]{\hspace*{-12pt} \raisebox{-3pt}{\footnotesize $0$}}
		\psfrag{0.1}{}
		\psfrag{0.2}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.2$}}
		\psfrag{0.3}{}
		\psfrag{0.4}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.4$}}
		\psfrag{0.5}{}
		\psfrag{0.6}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.6$}}
		\psfrag{0.7}{}
		\psfrag{0.8}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.8$}}
		\psfrag{0.9}{}
		\psfrag{1}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $1$}}
		\psfrag{a1}[cr][cr]{\raisebox{-3pt}{\footnotesize $1$}}
		\psfrag{3}[cr][cr]{\raisebox{-3pt}{\footnotesize $3$}}
		\psfrag{5}[cr][cr]{\raisebox{-3pt}{\footnotesize $5$}}
		\psfrag{domain}[Bc][Bc]{\raisebox{-7pt}{spatial domain $\bbX$}}
		\psfrag{coefficient}[bc][tc]{\raisebox{-24pt}{$\jumpCoeff (\stochVar, \spaceVar)$}}
		}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.495\textwidth}
		\centering
		\psfragfig[width=0.47\textwidth]{./pictures/coefficientSamples/alternatingExponential/alternatingExponential-Sample-2}{
		\psfrag{0}[Bc][Bc]{\hspace*{-10pt}\raisebox{-3pt}{\footnotesize $0$}}
		\psfrag{0.1}{}
		\psfrag{0.2}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.2$}}
		\psfrag{0.3}{}
		\psfrag{0.4}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.4$}}
		\psfrag{0.5}{}
		\psfrag{0.6}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.6$}}
		\psfrag{0.7}{}
		\psfrag{0.8}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.8$}}
		\psfrag{0.9}{}
		\psfrag{1}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $1$}}
		\psfrag{a1}[cr][cr]{\raisebox{-3pt}{\footnotesize $1$}}
		\psfrag{3}[cr][cr]{\raisebox{-3pt}{\footnotesize $3$}}
		\psfrag{5}[cr][cr]{\raisebox{-3pt}{\footnotesize $5$}}
		\psfrag{domain}[Bc][Bc]{\raisebox{-7pt}{spatial domain $\bbX$}}
		\psfrag{coefficient}[bc][tc]{\raisebox{-24pt}{$\jumpCoeff (\stochVar, \spaceVar)$}}
		}
	\end{subfigure}
	\caption{Two samples of the alternating jump field with an exponential Gaussian random field.}
	\label{fig:alternatingExponential_samples}
\end{figure}

==> pictures/coefficientSamples/inclusionField.tex <==
\begin{figure}[h!tbp]
	\centering
	\begin{subfigure}[b]{0.495\textwidth}
		\centering
		\psfragfig[width=0.47\textwidth]{./pictures/coefficientSamples/inclusionField/inclusionField-Sample-1}{
		\psfrag{0}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0$}}
		\psfrag{0.1}{}
		\psfrag{0.2}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.2$}}
		\psfrag{0.3}{}
		\psfrag{0.4}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.4$}}
		\psfrag{0.5}{}
		\psfrag{0.6}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.6$}}
		\psfrag{0.7}{}
		\psfrag{0.8}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.8$}}
		\psfrag{0.9}{}
		\psfrag{1}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $1$}}
		\psfrag{e-2}[cr][cr]{\footnotesize $10^{-2}$}
		\psfrag{e0}[cr][cr]{\footnotesize $10^{0}$}
		\psfrag{e2}[cr][cr]{\footnotesize $10^{2}$}
		\psfrag{domain}[Bc][Bc]{\raisebox{-7pt}{spatial domain $\bbX$}}
		\psfrag{coefficient}[bc][tc]{\raisebox{+2pt}{$\jumpCoeff (\stochVar, \spaceVar)$}}
		}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.495\textwidth}
		\centering
		\psfragfig[width=0.47\textwidth]{./pictures/coefficientSamples/inclusionField/inclusionField-Sample-2}{
		\psfrag{0}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0$}}
		\psfrag{0.1}{}
		\psfrag{0.2}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.2$}}
		\psfrag{0.3}{}
		\psfrag{0.4}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.4$}}
		\psfrag{0.5}{}
		\psfrag{0.6}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.6$}}
		\psfrag{0.7}{}
		\psfrag{0.8}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $0.8$}}
		\psfrag{0.9}{}
		\psfrag{1}[Bc][Bc]{\raisebox{-3pt}{\footnotesize $1$}}
		\psfrag{e-2}[cr][cr]{\footnotesize $10^{-2}$}
		\psfrag{e0}[cr][cr]{\footnotesize $10^{0}$}
		\psfrag{e2}[cr][cr]{\footnotesize $10^{2}$}
		\psfrag{domain}[Bc][Bc]{\raisebox{-7pt}{spatial domain $\bbX$}}
		\psfrag{coefficient}[bc][tc]{\raisebox{+4pt}{$\jumpCoeff (\stochVar, \spaceVar)$}}
		}
	\end{subfigure}
	\caption{Two realizations of the jump field with random inclusions.}
	\label{fig:inclusionField_samples}
\end{figure}

==> pictures/convergenceResults/convergenceAlternating.tex <==
\begin{figure}[h!tbp]
	\centering
	\begin{subfigure}[b]{.49\textwidth}
		\centering
		\psfragfig[width=.49\textwidth]{./pictures/convergenceResults/alternatingExponential/L1-error_vs_invStepSize}{
		\psfrag{95confInt.}{\tiny $95\%$ conf. interval}
		\psfrag{suppLineSlope0.93}{\tiny supp. line with slope $0.93$}
		\psfrag{FV}{\tiny equidistant finite volumes}
		\psfrag{JAFV}{\tiny jump-adaptive finite volumes}
		\psfrag{JAWCFV}{\tiny jump-adaptive wave-cell finite volumes}
		}
		\caption{Pathwise $L^{1}$ error.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{.49\textwidth}
		\centering
		\psfragfig[width=.49\textwidth]{./pictures/convergenceResults/alternatingExponential/L2-error_vs_invStepSize}{
		\psfrag{95confInt.}{\tiny $95\%$ conf. interval}
		\psfrag{suppLineSlope0.65}{\tiny supp. line with slope $0.65$}
		\psfrag{FV}{\tiny equidistant finite volumes}
		\psfrag{JAFV}{\tiny jump-adaptive finite volumes}
		\psfrag{JAWCFV}{\tiny jump-adaptive wave-cell finite volumes}
		}
		\caption{Pathwise $L^{2}$ error.}
	\end{subfigure}
	\caption{Strong error for the alternating jump field with exponential Gaussian random field. The error estimation is based on $50$ samples.}
	\label{fig:alternatingExponential_errorVsStepSize}
\end{figure}

==> pictures/convergenceResults/convergenceInclusion.tex <==
\begin{figure}[h!tbp]
	\centering
	\begin{subfigure}[b]{.49\textwidth}
		\psfragfig[width=.49\textwidth]{./pictures/convergenceResults/inclusionField/L1-error_vs_invStepSize}{
		\psfrag{95confInt.}{\tiny $95\%$ conf. interval}
		\psfrag{suppLineSlope0.65}{\tiny supp. line with slope $0.65$}
		\psfrag{linFitSlope0.37}{\tiny supp. line with slope $0.37$}
		\psfrag{FV}{\tiny equidistant finite volumes}
		\psfrag{JAFV}{\tiny jump-adaptive finite volumes}
		\psfrag{JAWCFV}{\tiny jump-adaptive wave-cell finite volumes}
		}
		\caption{Pathwise $L^{1}$ error.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{.49\textwidth}
		\psfragfig[width=.49\textwidth]{./pictures/convergenceResults/inclusionField/L2-error_vs_invStepSize}{
		\psfrag{95confInt.}{\tiny $95\%$ conf. interval}
		\psfrag{suppLineSlope0.51}{\tiny supp. line with slope $0.51$}
		\psfrag{linFitSlope0.11}{\tiny supp. line with slope $0.11$}
		\psfrag{FV}{\tiny equidistant finite volumes}
		\psfrag{JAFV}{\tiny jump-adaptive finite volumes}
		\psfrag{JAWCFV}{\tiny jump-adaptive wave-cell finite volumes}
		}
		\caption{Pathwise $L^{2}$ error.}
	\end{subfigure}
	\caption{Strong error for the stochastic jump field with random inclusions based on $100$ samples.}
	\label{fig:inclusionField}
\end{figure}

==> pictures/convergenceResults/convergencePoisson.tex <==
\begin{figure}[h!tbp]
	\centering
	\begin{subfigure}[b]{.49\textwidth}
		\centering
		\psfragfig[width=.49\textwidth]{./pictures/convergenceResults/PoissonSquaredExponential/L1-error_vs_invStepSize}{
		\psfrag{95confInt.}{\tiny $95\%$ conf. interval}
		\psfrag{suppLineSlope1.06}{\tiny supp. line with slope $1.06$}
		\psfrag{FV}{\tiny equidistant finite volumes}
		\psfrag{JAFV}{\tiny jump-adaptive finite volumes}
		\psfrag{JAWCFV}{\tiny jump-adaptive wave-cell finite volumes}
		}
		\caption{Pathwise $L^{1}$ error.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{.49\textwidth}
		\centering
		\psfragfig[width=.49\textwidth]{./pictures/convergenceResults/PoissonSquaredExponential/L2-error_vs_invStepSize}{
		\psfrag{95confInt.}{\tiny $95\%$ conf. interval}
		\psfrag{suppLineSlope0.66}{\tiny supp. line with slope $0.66$}
		\psfrag{FV}{\tiny equidistant finite volumes}
		\psfrag{JAFV}{\tiny jump-adaptive finite volumes}
		\psfrag{JAWCFV}{\tiny jump-adaptive wave-cell finite volumes}
		}
		\caption{Pathwise $L^{2}$ error.}
%		\label{sfig:Poisson_L2}
	\end{subfigure}
	\caption{Strong error for the Poisson jump field with squared-exponential Gaussian random field estimated with $50$ samples.}
	\label{fig:PoissonSquaredExponential}
\end{figure}

==> pictures/explicitVsImplicit/minStepSize_L1.tex <==
\begin{figure}[htbp!]
	\begin{subfigure}{.325\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/explicitVsImplicit/minStepSize_L1/delta_1e-2}{
		\psfrag{forwardEuler}{\tiny Forward Euler}
		\psfrag{backwardEuler}{\tiny Backward Euler}
		}
		\caption{$\delta = 10^{-2}$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.325\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/explicitVsImplicit/minStepSize_L1/delta_1e-3}{
		\psfrag{forwardEuler}{\tiny Forward Euler}
		\psfrag{backwardEuler}{\tiny Backward Euler}
		}
		\caption{$\delta = 10^{-3}$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.325\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/explicitVsImplicit/minStepSize_L1/delta_1e-4}{
		\psfrag{forwardEuler}{\tiny Forward Euler}
		\psfrag{backwardEuler}{\tiny Backward Euler}
		}
		\caption{$\delta = 10^{-4}$.}
	\end{subfigure}
	\caption{Time to error plot of the forward Euler and backward Euler time discretization of the jump-adapted finite volume approximation for different jump distances $\delta > 0$.}
	\label{fig:explciitVsImplicit_DeltaX}
\end{figure}

==> pictures/explicitVsImplicit/waveSpeed_L1.tex <==
\begin{figure}[h!tbp]
	\centering
	\begin{subfigure}[b]{.325\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/explicitVsImplicit/waveSpeed_L1/timeToError_maxCoeff-20}{
		\psfrag{forwardEuler}{\tiny Forward Euler}
		\psfrag{backwardEuler}{\tiny Backward Euler}
		}
		\caption{$\kappa = 0.3$, $P_1 = 10.5$, $P_2 = 20$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{.325\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/explicitVsImplicit/waveSpeed_L1/timeToError_maxCoeff-50}{
		\psfrag{forwardEuler}{\tiny Forward Euler}
		\psfrag{backwardEuler}{\tiny Backward Euler}
		}
		\caption{$\kappa = 0.3$, $P_1 = 1$, $P_2 = 50$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{.325\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/explicitVsImplicit/waveSpeed_L1/timeToError_maxCoeff-50_sin-1}{
		\psfrag{forwardEuler}{\tiny Forward Euler}
		\psfrag{backwardEuler}{\tiny Backward Euler}
		}
		\caption{$\kappa = 1$, $P_1 = 1$, $P_2 = 50$.}
		\label{sfig:waveSpeed_50_sin1}
	\end{subfigure}
	\caption{Time to error plots of the forward and backward Euler scheme with a jump-adapted finite volume discretization for different values of $\kappa$ and $P_1, P_2$.}
	\label{fig:explicitVsImplicit_waveSpeed}
\end{figure}

==> pictures/jumpInfluence/jumpDistance_jump-down_L1.tex <==
\begin{figure}[htbp!]
	\begin{subfigure}{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/jumpInfluence/jumpDistance_jump-down_L1/delta_2-4}{
		\psfrag{supportLine0.98}{\tiny supp. line with slope $0.98$}
		\psfrag{linearFit0.67}{\tiny lin. fit with slope $0.67$}
		\psfrag{nonAdaptedL1Error}{\tiny non-adapted $L^{1}$ error}
		\psfrag{supportLine1.04}{\tiny supp. line with slope $1.04$}
		\psfrag{linearFit0.71}{\tiny lin. fit with slope $0.71$}
		\psfrag{jump-adaptedL1Error}{\tiny adapted $L^{1}$ error}
		}
		\caption{$\delta = 2^{-4}$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/jumpInfluence/jumpDistance_jump-down_L1/delta_2-6}{
		\psfrag{supportLine1.03}{\tiny supp. line with slope $1.03$}
		\psfrag{linearFit0.73}{\tiny lin. fit with slope $0.73$}
		\psfrag{nonAdaptedL1Error}{\tiny non-adapted $L^{1}$ error}
		\psfrag{supportLine1.03}{\tiny supp. line with slope $1.03$}
		\psfrag{linearFit0.48}{\tiny lin. fit with slope $0.48$}
		\psfrag{jump-adaptedL1Error}{\tiny adapted $L^{1}$ error}
		}
		\caption{$\delta = 2^{-6}$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/jumpInfluence/jumpDistance_jump-down_L1/delta_2-8}{
		\psfrag{supportLine0.79}{\tiny supp. line with slope $0.79$}
		\psfrag{linearFit0.85}{\tiny lin. fit with slope $0.85$}
		\psfrag{nonAdaptedL1Error}{\tiny non-adapted $L^{1}$ error}
		\psfrag{supportLine0.91}{\tiny supp. line with slope $0.91$}
		\psfrag{linearFit0.16}{\tiny lin. fit with slope $0.16$}
		\psfrag{jump-adaptedL1Error}{\tiny adapted $L^{1}$ error}
		}
		\caption{$\delta = 2^{-8}$.}
	\end{subfigure}
	\caption{Convergence rates for $a(x) = P^{\text{down}}(x)$ and various $\delta$.}
	\label{fig:jumpDistance_jumpDown}
\end{figure}

==> pictures/jumpInfluence/jumpDistance_jump-up_L1.tex <==
\begin{figure}[htbp!]
	\begin{subfigure}{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/jumpInfluence/jumpDistance_jump-up_L1/delta_2-4}{
		\psfrag{supportLine0.75}{\tiny supp. line with slope $0.75$}
		\psfrag{linearFit0.64}{\tiny lin. fit with slope $0.64$}
		\psfrag{nonAdaptedL1Error}{\tiny non-adapted $L^{1}$ error}
		\psfrag{supportLine0.85}{\tiny supp. line with slope $0.85$}
		\psfrag{linearFit0.59}{\tiny lin. fit with slope $0.59$}
		\psfrag{jump-adaptedL1Error}{\tiny adapted $L^{1}$ error}
		}
		\caption{$\delta = 2^{-4}$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/jumpInfluence/jumpDistance_jump-up_L1/delta_2-6}{
		\psfrag{supportLine0.72}{\tiny supp. line with slope $0.72$}
		\psfrag{linearFit0.75}{\tiny lin. fit with slope $0.75$}
		\psfrag{nonAdaptedL1Error}{\tiny non-adapted $L^{1}$ error}
		\psfrag{supportLine0.73}{\tiny supp. line with slope $0.73$}
		\psfrag{linearFit0.61}{\tiny lin. fit with slope $0.61$}
		\psfrag{jump-adaptedL1Error}{\tiny adapted $L^{1}$ error}
		}
		\caption{$\delta = 2^{-6}$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/jumpInfluence/jumpDistance_jump-up_L1/delta_2-8}{
		\psfrag{supportLine1.05}{\tiny supp. line with slope $1.05$}
		\psfrag{linearFit0.63}{\tiny lin. fit with slope $0.63$}
		\psfrag{nonAdaptedL1Error}{\tiny non-adapted $L^{1}$ error}
		\psfrag{supportLine0.83}{\tiny supp. line with slope $0.83$}
		\psfrag{linearFit0.91}{\tiny lin. fit with slope $0.91$}
		\psfrag{jump-adaptedL1Error}{\tiny adapted $L^{1}$ error}
		}
		\caption{$\delta = 2^{-8}$.}
	\end{subfigure}
	\caption{Convergence rates for $a(x) = P^{\text{up}}(x)$ and various $\delta$.}
	\label{fig:jumpDistance_jumpUp}
\end{figure}

==> pictures/jumpInfluence/numberOfJumps_L1.tex <==
\begin{figure}[htbp!]
	\begin{subfigure}{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/jumpInfluence/numberOfJumps_L1/numJumps-4}{
		\psfrag{supportLine0.92}{\tiny supp. line with slope $0.92$}
		\psfrag{linearFit0.62}{\tiny lin. fit with slope $0.62$}
		\psfrag{nonAdaptedL1Error}{\tiny non-adapted $L^{1}$ error}
		\psfrag{supportLine0.87}{\tiny supp. line with slope $0.87$}
		\psfrag{linearFit0.66}{\tiny lin. fit with slope $0.66$}
		\psfrag{jump-adaptedL1Error}{\tiny adapted $L^{1}$ error}
		}
		\caption{$\numberOfJumps = 4$ jumps.}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/jumpInfluence/numberOfJumps_L1/numJumps-16}{
		\psfrag{supportLine0.72}{\tiny supp. line with slope $0.72$}
		\psfrag{linearFit0.55}{\tiny lin. fit with slope $0.55$}
		\psfrag{nonAdaptedL1Error}{\tiny non-adapted $L^{1}$ error}
		\psfrag{supportLine0.69}{\tiny supp. line with slope $0.69$}
		\psfrag{linearFit0.5}{\tiny lin. fit with slope $0.5$}
		\psfrag{jump-adaptedL1Error}{\tiny adapted $L^{1}$ error}
		}
		\caption{$\numberOfJumps = 16$ jumps.}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.32\textwidth}
		\psfragfig[width=.32\textwidth]{./pictures/jumpInfluence/numberOfJumps_L1/numJumps-64}{
		\psfrag{supportLine0.55}{\tiny supp. line with slope $0.55$}
		\psfrag{linearFit0.4}{\tiny lin. fit with slope $0.4$}
		\psfrag{nonAdaptedL1Error}{\tiny non-adapted $L^{1}$ error}
		\psfrag{supportLine0.53}{\tiny supp. line with slope $0.53$}
		\psfrag{linearFit0.36}{\tiny lin. fit with slope $0.36$}
		\psfrag{jump-adaptedL1Error}{\tiny adapted $L^{1}$ error}
		}
		\caption{$\numberOfJumps = 64$ jumps.}
		\label{sfig:64jumps}
	\end{subfigure}
	\caption{Convergence rates for $a(x) = P(x)$ with varying number of jumps.}
	\label{fig:numberOfJumps}
\end{figure}
